NeRF-MAE: Masked AutoEncoders for Self-Supervised 3D Representation Learning for Neural Radiance Fields

Neural fields excel in computer vision and robotics due to their ability to understand the 3D visual world such as inferring semantics, geometry, and dynamics. Given the capabilities of neural fields in densely representing a 3D scene from 2D images, we ask the question: Can we scale their self-supervised pretraining, specifically using masked autoencoders, to generate effective 3D representations from posed RGB images. Owing to the astounding success of extending transformers to novel data modalities, we employ standard 3D Vision Transformers to suit the unique formulation of NeRFs. We leverage NeRF's volumetric grid as a dense input to the transformer, contrasting it with other 3D representations such as pointclouds where the information density can be uneven, and the representation is irregular. Due to the difficulty of applying masked autoencoders to an implicit representation, such as NeRF, we opt for extracting an explicit representation that canonicalizes scenes across domains by employing the camera trajectory for sampling. Our goal is made possible by masking random patches from NeRF's radiance and density grid and employing a standard 3D Swin Transformer to reconstruct the masked patches. In doing so, the model can learn the semantic and spatial structure of complete scenes. We pretrain this representation at scale on our proposed curated posed-RGB data, totaling over 1.8 million images. Once pretrained, the encoder is used for effective 3D transfer learning. Our novel self-supervised pretraining for NeRFs, NeRF-MAE, scales remarkably well and improves performance on various challenging 3D tasks. Utilizing unlabeled posed 2D data for pretraining, NeRF-MAE significantly outperforms self-supervised 3D pretraining and NeRF scene understanding baselines on Front3D and ScanNet datasets with an absolute performance improvement of over 20% AP50 and 8% AP25 for 3D object detection.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}

==> sec/7_suppl_arXiv.tex <==
\clearpage



\begin{center}
\vspace{0.2cm}
    {\Large \textbf{ NeRF-MAE: Masked AutoEncoders for Self Supervised 3D Representation Learning for Neural Radiance Fields \\[0.5em] --- Supplementary Material ---}}\\[2em] % [1em] adds some vertical space after the title

    Anonymous ECCV 2024 Submission \\[1em]
    Paper ID \#12306 
\end{center}
% \begin{strip}
% \begin{center}
% \vspace{-5ex}
% \textbf{\Large \bf
% % Panoptic Segmentation in the Bird's Eye View
% % Learning and Aggregating Lane Graphs for Urban Automated Driving
% Supplementary material for NeRF-MAE: Masked AutoEncoders for Self Supervised 3D Representation Learning for Neural Radiance Fields
% } \\
% \vspace{2ex}

% \Large{\bf Supplementary Material}\\
% \vspace{0.4cm}
% \large{
% Nick~Heppert,~
% Muhammad~Zubair~Irshad,~
% Sergey~Zakharov,~
% Katherine~Liu,\\
% Rares~Andrei~Ambrus,~
% Jeannette~Bohg,~
% Abhinav~Valada,~
% Thomas~Kollar
% }
% \end{center}
% \end{strip}

% \twocolumn[{%
% \renewcommand\twocolumn[1][]{#1}%
% \maketitlesupplementary
\setcounter{page}{1}
\setcounter{section}{0} % Reset section counter to 0
% \setcounter{figure}{10} % Reset section counter to 0
% \setcounter{table}{5} % Reset section counter to 0

\setcounter{figure}{0} % Reset section counter to 0
\setcounter{table}{0} % Reset section counter to 0

\renewcommand{\thetable}{S.\arabic{table}}
\renewcommand{\thefigure}{S.\arabic{figure}}
\renewcommand{\thesection}{\Alph{section}} % Section counter format: A, B, C, ...
% \makeatletter

This supplementary material is divided into 5 sections. First, we provide details regarding network architecture and number of parameters in Section~\ref{sec:architecture_details}. Second, we provide an overview of implementation details in Section~\ref{sec:implementation_details}. This is followed by a discussion on additional experimental analysis in Section~\ref{sec:add_experiments}. We provide an overview of pretraining datasets in Section~\ref{sec:pretraining_datasets} and discuss compute resources required to pretrain our representation in Section~\ref{sec:compute_resources}. Lastly, we discuss limitations and future work in Section~\ref{sec:future_work}.


\input{sec/supplementary/s1_architecture}
\input{sec/supplementary/s3_implementation}
\input{sec/supplementary/s4_additional_experiment_analysis}
\input{sec/supplementary/s5_pretraining_dataset}
\input{sec/supplementary/s2_compute_resources}
\input{sec/supplementary/s6_future_work}

% This supplementary material is divided into 5 sections. First, we provide details regarding network architecture and number of parameters in Section~\ref{sec:architecture_details}. Second, we provide an overview of implementation details in Section~\ref{sec:implementation_details}. This is followed by a discussion on additional experimental analysis in Section~\ref{sec:add_experiments}. We provide an overview of pretraining datasets in Section~\ref{sec:pretraining_datasets} and discuss compute resources required to pretrain our representation in Section~\ref{sec:compute_resources}. Lastly, we discuss limitations and future work in Section~\ref{sec:future_work}.


% \input{sec/supplementary/s1_architecture}
% \input{sec/supplementary/s3_implementation}
% \input{sec/supplementary/s4_additional_experiment_analysis}
% \input{sec/supplementary/s5_pretraining_dataset}
% \input{sec/supplementary/s2_compute_resources}
% \input{sec/supplementary/s6_future_work}

% \section{Rationale}
% \label{sec:rationale}
% % 
% Having the supplementary compiled together with the main paper means that:
% % 
% \begin{itemize}
% \item The supplementary can back-reference sections of the main paper, for example, we can refer to \cref{sec:intro};
% \item The main paper can forward reference sub-sections within the supplementary explicitly (e.g. referring to a particular experiment); 
% \item When submitted to arXiv, the supplementary will already included at the end of the paper.
% \end{itemize}
% % 
% To split the supplementary pages from the main paper, you can use \href{https://support.apple.com/en-ca/guide/preview/prvw11793/mac#:~:text=Delete%20a%20page%20from%20a,or%20choose%20Edit%20%3E%20Delete).}{Preview (on macOS)}, \href{https://www.adobe.com/acrobat/how-to/delete-pages-from-pdf.html#:~:text=Choose%20%E2%80%9CTools%E2%80%9D%20%3E%20%E2%80%9COrganize,or%20pages%20from%20the%20file.}{Adobe Acrobat} (on all OSs), as well as \href{https://superuser.com/questions/517986/is-it-possible-to-delete-some-pages-of-a-pdf-document}{command line tools}.

\clearpage

==> tables/depth_ablation.tex <==
\begin{minipage}{.46\linewidth}
\scriptsize
\setlength{\tabcolsep}{0.6em}
\centering


% \resizebox{0.45\textwidth}{!}{%
\begin{tabular}{cccc}
\toprule
\multicolumn{4}{c}{\textit{Rendered Depth Quantitative Evaluation}}\\
\cmidrule(lr){1-4}
Method & PSNR& \textbf{AbsRel}$\downarrow$ & \textbf{RMSE}$\downarrow$ \\

\midrule
\multicolumn{1}{c|}{\multirow{ 2}{*}{Instant-NGP}}  & \multicolumn{1}{c|}{21} & 0.459 & 0.995  \\
\multicolumn{1}{c|}{} & \multicolumn{1}{c|}{32} & \textbf{0.164} & \textbf{0.318} \\
\bottomrule
\end{tabular}
% }

% \caption{\textbf{Effect of skip connections in the decoder} during pretraining showing NeRF-MAE with skip connection helps learn better representations for downstream tasks}
% \label{tab:skip_ablation}
% \end{table}

\end{minipage}

==> tables/pretraining_mae_comparisons.tex <==
% \begin{table}[htb!]
% \centering
% \scriptsize
% % \resizebox{0.45\textwidth}{!}{%
% \begin{tabularx}{\columnwidth}{ccccCC}
% \toprule
% \multicolumn{3}{c}{MAE Baselines} & \multicolumn{2}{c}{Metrics}\\
% \cmidrule(lr){1-3}\cmidrule(lr){4-5}
% Approach & 3D Backbone & Full Ann. & \multicolumn{2}{c}{ScanNet} \\
% \midrule
% & & & \textbf{Recall50} & \textbf{AP50} \\
% \midrule
% DepthContrast & VoteNet &  \textcolor{teal}{\checkmark} &+4.2 & +1.7 \\
% \midrule
% NeRF-MAE (Ours) & NeRF-RPN & \textcolor{falured}{\xmark} & \textbf{+7.2} & \textbf{+3.0} \\
% \bottomrule
% \end{tabularx}
% % }
% \caption{\textbf{Quantitative comparisons} showing our approach's relative improvement number vs other masked auto-encoder approaches where VoteNet requires all annotations such as instance masks and mean class sizes}
% \vspace{-8pt}
% \label{tab:pretraining_mae_comparisons}
% \end{table}
% \vspace{-5pt}
\begin{table}[h!]
\centering
\scriptsize
% \resizebox{0.45\textwidth}{!}{%
\begin{tabularx}{\columnwidth}{ccCCC|CCC}
\toprule
% \multicolumn{2}{c}{MAE Baselines} & \multicolumn{6}{c}{Metrics}\\
Approach & Full Ann. & \multicolumn{6}{c}{Metrics on ScanNet test-set} \\
\cmidrule(lr){1-2}\cmidrule(lr){3-8}
% \midrule
& & \multicolumn{3}{c}{\textbf{Recall50}} & \multicolumn{3}{c}{\textbf{AP50}} \\
\midrule

& & \textbf{S} & \textbf{PT} & \textbf{Diff.} & \textbf{S} & \textbf{PT} & \textbf{Diff.} \\

\midrule
DepthContrast~\citedepthcontrast &  \textcolor{teal}{\checkmark} & 7.5 & 11.7 & +4.2 & 2.4 & 4.1 & +1.7 \\
\midrule
NeRF-MAE (Ours) & \textcolor{falured}{\xmark} & 32.3  & 39.5 & \textbf{+7.2}& 14.0 & 17.0 & \textbf{+3.0}\\
\bottomrule
\end{tabularx}
% }
\caption{\textbf{Quantitative comparison} showing our approach's superior result vs strong MAE baseline where~\citedepthcontrast{} uses VoteNet requiring full annotations such as instance masks and mean class size.~\textbf{S} denotes starting from scratch and~\textbf{PT} denotes pretrained.}
% \vspace{-8pt}
\label{tab:pretraining_mae_comparisons}
\end{table}

==> tables/voxel_grid_super_resolution.tex <==
\begin{table}[t!]
\centering
\setlength{\tabcolsep}{2.5pt}
\scriptsize
\begin{tabularx}{\columnwidth}{c|CC|CC}

\toprule

& \multicolumn{2}{c}{$256^{3}$} & \multicolumn{2}{c}{$384^{3}$}\\
\cmidrule(lr){1-2}
\cmidrule(lr){2-3} \cmidrule(lr){4-5}
 Method & \textbf{PSNR}$\uparrow$& \textbf{MSE} $\downarrow$&  \textbf{PSNR}$\uparrow$& \textbf{MSE} $\downarrow$ \\ 
% \midrule
\hline 

NeRF-RPN*~\cite{hu2023nerf} & 16.25 &0.024 & 16.08 &0.025 \\
NeRF-MAE(Ours) &\cellcolor{tabfirst}17.27 &\cellcolor{tabfirst}0.019 &\cellcolor{tabfirst}17.34 &\cellcolor{tabfirst}0.019\\
\bottomrule
\end{tabularx}

\caption{\textbf{Voxel super-resolution quantitative results:} showing superior performance of our method vs NeRF-RPN~\cite{hu2023nerf}. * denotes we add a task-specific head to NeRF-RPN's Swin-S encoder.}

% \vspace{-12pt}
\label{tab:voxel_super_resolution}
\end{table}

==> tables/voxel_labelling_task.tex <==
\begin{table}[t!]
\centering
  \setlength{\tabcolsep}{1.5pt}
 \scriptsize
\begin{tabularx}{\columnwidth}{c|CC|CC}
\toprule

& \multicolumn{2}{c}{Front3D~\cite{fu20213d}} & \multicolumn{2}{c}{HM3D~\cite{ramakrishnan2021hm3d}} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5}
Metrics & NeRF-RPN*~\cite{hu2023nerf} & NeRF-MAE& NeRF-RPN*~\cite{hu2023nerf} & NeRF-MAE \\
% \midrule
\hline
\textbf{mIOU}$\uparrow$  & 0.249 & \cellcolor{tabfirst}0.345 & 0.109 & \cellcolor{tabfirst}0.186 \\
\textbf{mAcc}$\uparrow$ & 0.338 & \cellcolor{tabfirst}0.450 & 0.160 & \cellcolor{tabfirst}0.264 \\
\textbf{Acc}$\uparrow$ & 0.730 & \cellcolor{tabfirst}0.810 & 0.510 & \cellcolor{tabfirst}0.581 \\
\bottomrule
% \end{tabular}
\end{tabularx}
\caption{\textbf{Semantic voxel-labelling results:} showing superior performance of our method vs NeRF-RPN~\cite{hu2023nerf}. * denotes we add a task-specific head to NeRF-RPN's Swin-S encoder.}
% \vspace{-14pt}
\label{tab:voxel_labelling}
\end{table}
